Detecting Anomalous User Behavior Using an Extended Isolation Forest Algorithm: An Enterprise Case Study

Anomalous user behavior detection is the core component of many information security systems, such as intrusion detection, insider threat detection and authentication systems. Anomalous behavior will raise an alarm to the system administrator and can be further combined with other information to determine whether it constitutes an unauthorised or malicious use of a resource. This paper presents an anomalous user behaviour detection framework that applies an extended version of Isolation Forest algorithm. Our method is fast and scalable and does not require example anomalies in the training data set. We apply our method to an enterprise dataset. The experimental results show that the system is able to isolate anomalous instances from the baseline user model using a single feature or combined features.

==> background.tex <==
\section{Background}
\label{sec:background}



==> iforest_desc.tex <==
\subsection{Isolation Forest}
\label{if}

Isolation forest (iForest) \cite{liu2008isolation} is an anomaly detection algorithm.
The algorithm utilises the observation that if a dataset is organised
into a binary search tree, anomalies are more likely to be inserted
at a lesser depth in a tree, compared to non-anomalous values.
For a given dataset, the algorithm takes $n$ random samples of size $m$.
For each random sample, a binary search tree is contructed, randomly selecting
a dimension and partition point for each comparison node in the tree.
To calculate the anomaly score of a new data point, it is inserted
into to each of the $n$ random trees. The anomaly score is derived
from the mean insertion depth across all of the trees.

Isolation forest has a number of advantages as an anomaly detection algorithm:
\begin{itemize}
\item
It requires relatively small samples from large datasets to derive an anomaly detection
function. This makes it fast and scalable.
\item
It does not require example anomalies in the training data set.
\item
Its distance threshold for determining anomalies is based on tree depth,
which is independent of the scaling of the data set dimensions.
\end{itemize}

\begin{figure}
\subfigure[]{\includegraphics[width=0.45\textwidth]{iforest_example_normal.png}}
\subfigure[]{\includegraphics[width=0.45\textwidth]{iforest_tree.png}}

\caption{(a) In this example dataset, a randomly constructed binary search
tree isolates the anomalous value (17,17) (shown in red) in just one division,
whereas the medoid value (7,13) (shown in blue) is isolated in five random divisions.
(b) The anomaly has a tree depth of 1, compared to 5 for the medoid point.}
\label{fig:iforestexample}
\end{figure}


\subsection{Extended Isolation Forest to categorical data}
\label{if_extend}

Isolation forest was originally proposed for datasets with continuous dimensions.
In this paper we extend the algorithm to consider categorical data.
Our method only requires that for each categorical dimension, values
have an ordering. The ordering may be arbitrary. Each value is then
mapped to a numeric value, based on its ordering.

For example the values \emph{true} and \emph{false} may be mapped
to $\mathit{false} = 0$, $\mathit{true} = 1$.

Having mapped the categorical values to numeric values, the
categorical dimensions can be treated the same way as the
numeric dimensions in the isolation forest algorithm.

